Graph Pattern Matching in GQL and SQL/PGQ

As graph databases become widespread, JTC1 -- the committee in joint charge of information technology standards for the International Organization for Standardization (ISO), and International Electrotechnical Commission (IEC) -- has approved a project to create GQL, a standard property graph query language. This complements a project to extend SQL with a new part, SQL/PGQ, which specifies how to define graph views over an SQL tabular schema, and to run read-only queries against them. Both projects have been assigned to the ISO/IEC JTC1 SC32 working group for Database Languages, WG3, which continues to maintain and enhance SQL as a whole. This common responsibility helps enforce a policy that the identical core of both PGQ and GQL is a graph pattern matching sub-language, here termed GPML. The WG3 design process is also analyzed by an academic working group, part of the Linked Data Benchmark Council (LDBC), whose task is to produce a formal semantics of these graph data languages, which complements their standard specifications. This paper, written by members of WG3 and LDBC, presents the key elements of the GPML of SQL/PGQ and GQL in advance of the publication of these new standards.

==> concl.tex <==
To be done last

==> qt.tex <==
A quick tour (to be written after the detailed description) (Filip)

[Compare: proposed summary of concepts of graph pattern matching in SQL/PGQ]

[Actually better this one https://docs.google.com/document/d/175cNEmVQI3AgNUWeGG7DKaQp1hiN4Gbtxiab5kwnbYE/edit]


A few basic examples of PGQ patterns based on the example from Section 2

TEAM: Alin

